Elastically safeguarded augmented Lagrangian methods

We investigate, theoretically and numerically, a class of elastically safeguarded augmented Lagrangian methods for nonlinear optimization problems with inequality and equality constraints. Safeguarded augmented Lagrangian methods are known to exhibit substantially stronger global convergence guarantees than their non-safeguarded counterparts, making them attractive in practice. A persistent limitation, however, is that existing methods rely on a fixed safeguard, whose a priori selection can be difficult and inherently limits adaptivity, e.g., with respect to problem scaling. We propose an adaptive safeguarding mechanism that allows the safeguard to grow dynamically, overcoming these drawbacks while preserving the desirable global convergence properties of variants with a fixed safeguard. We further establish complexity bounds in terms of worst-case iteration counts. Numerical experiments comparing ALGENCAN, a state-of-the-art solver with rigid safeguard, against an elastically safeguarded variant thereof confirm that elastic safeguarding yields consistent practical benefits.

==> preamble.tex <==
\usepackage{fullpage}
\usepackage{multirow}

\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{nicefrac}
\usepackage{enumitem}
\usepackage{xcolor}
\definecolor{cb2blue}{RGB}{55,126,184}
\definecolor{cb2green}{RGB}{77,175,74}
\definecolor{cb2red}{RGB}{228,26,28}
\definecolor{cb2orange}{RGB}{255,127,0}
\usepackage{graphicx}

\RequirePackage{doi}

\usepackage{cite}
\usepackage{hyperref}
\hypersetup{colorlinks,
	citecolor=cb2green,
	linkcolor=cb2blue,
	urlcolor=cb2red}

\usepackage[ruled,vlined,linesnumbered,algosection,algo2e]{algorithm2e} % Before cleveref

\usepackage[capitalize,noabbrev,nameinlink]{cleveref} % After hyperref

\newcommand{\includetikz}[1]{%
	\includegraphics{pics/#1}%
}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assum}[theorem]{Assumption}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

%commands
\newcommand{\emailLink}[1]{\href{mailto:#1}{#1}}
\newcommand{\orcidLink}[1]{\href{https://orcid.org/#1}{#1}}
\newcommand{\email}[1]{\textsc{email} \emailLink{#1}}
\newcommand{\orcid}[1]{\textsc{orcid} \orcidLink{#1}}
\newcommand{\amsmscLink}[1]{\href{http://www.ams.org/mathscinet/msc/msc2020.html?t=#1}{#1}}

\newcommand\blfootnote[1]{%
	\begingroup
	\renewcommand\thefootnote{}\footnote{#1}%
	\addtocounter{footnote}{-1}%
	\endgroup
}

% math commands
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}

\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\stt}{subject~to}
\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\norm}[1]{\Vert #1 \Vert}
\newcommand{\innprod}[2]{\langle #1,#2 \rangle}
\newcommand{\coloneqq}{:=}
\DeclareMathOperator{\diameter}{diam}
\DeclareMathOperator{\extent}{ext}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\newcommand{\Lag}{\mathcal{L}}
\newcommand{\AugLag}{\mathcal{L}^\textup{a}}
\newcommand{\safeYY}{Y_\textup{sg}}
\newcommand{\multYY}{Y_\textup{mul}}

\numberwithin{equation}{section}

\newcommand{\cbig}{c_{\rm{viol}}}
\newcommand{\cf}{c_{f}}
\newcommand{\cg}{c_{g}}
\newcommand{\ch}{c_{h}}
\newcommand{\cdiam}{c_{\rm D}}
\newcommand{\deltalow}{\delta_{\rm low}}
\newcommand{\feasmeas}{\mathcal{F}}
\newcommand{\pertfeasmeas}{\mathcal{P}}

\crefname{assum}{Assumption}{Assumptions}

\newcommand{\Ninnertol}{K}
\newcommand{\Niterout}{N_{\mathrm{out}}}
\newcommand{\Npenupdates}{N_{\mathrm{upd}}}
\newcommand{\Niterin}{N_{\mathrm{in}}}
\newcommand{\Nitertot}{N_{\mathrm{tot}}}
\newcommand{\citerin}{c_{\mathrm{in}}}

\newcommand{\ralgencan}{\textsc{ralm}}
\newcommand{\ealgencan}{\textsc{ealm}}
